Fee-Redistribution Smart Contracts for Transaction-Fee-Based Regime of Blockchains with the Longest Chain Rule

In this paper, we review the undercutting attacks in the transaction-fee-based regime of proof-of-work (PoW) blockchains with the longest chain fork-choice rule. Next, we focus on the problem of fluctuations in mining revenue and the mining gap - i.e., a situation, in which the immediate reward from transaction fees does not cover miners' expenditures. To mitigate these issues, we propose a solution that splits transaction fees from a mined block into two parts - (1) an instant reward for the miner of a block and (2) a deposit sent to one or more fee-redistribution smart contracts ($\mathcal{FRSC}$s) that are part of the consensus protocol. At the same time, these redistribution smart contracts reward the miner of a block with a certain fraction of the accumulated funds of the incoming fees over a predefined time. This setting enables us to achieve several interesting properties that are beneficial for the incentive stability and security of the protocol. With our solution, the fraction of Default-Compliant miners who strictly do not execute undercutting attacks is lowered from the state-of-the-art result of 66% to 30%.

==> sec/conclusion.tex <==
In this work, we focused on three problems related to transaction-fee-based regime of blockchains with the longest chain fork choice rule:
(1) the mining gap, (2) the possibility of undercutting attacks, and (3) the instability of mining rewards.
To mitigate these problems, we proposed the approach approximating a moving average based on the fee-redistributions smart contracts that accumulate a certain fraction of transaction fees and at the same time reward the miners from their reserves.
In this way, the miners are sufficiently rewarded even at the time of very low transaction fees, such as the beginning of the mining round, entering the mining protocol by new miners, market deviations, etc. 

Besides, our approach brings a higher tolerance to undercutting attacks, and increases the minimal threshold of \textsc{Default-Compliant} miner that strictly do not perform undercutting attack from 66\% reported in state-of-the-art to 30\%.


%The main motivation for this paper on how to solve possible bitcoin's future problem and a motivation for blockchains of future to consider this Proof of Concept into their design.
%This makes blockchains more resistant and reliable against security risk once being secured only based on transaction fees. \\
%
%Problem with too short contracts they will oscilate too much with blocks being found at different times (i.e. if 10min mean time block average can not be considered valid)

%\ih submissions are anonymous
%\section{Acknowledgments} 
%We are extremely grateful to Alexander Chepurnoy for early discussions and the idea of using multiple contracts.

==> sec/discussion.tex <==
\subsection{Contract-Drying Attack}
This is a new attack that might potentially occur in our scheme; however, it is the abusive attack aimed at attacking the functionality of our scheme and not on maximizing the profits of the adversary.
In this attack, the adversary aims at getting his reward only from $\mathcal{FRSC}$s and does not include transactions in the block (or includes only a number of them).
This might result in slow drying of the funds from $\mathcal{FRSC}$s and would mean less reward for future honest miners.
Moreover, the attacker can mine in well times of higher saturation of $\mathcal{FRSC}$s and after some time decide to switch off the mining.
This might cause a deterioration in profitability for honest miners, consequently leading to deteriorated security w.r.t., undercutting attacks.

The attacker can keep repeating this behavior, which would likely lead to increased transaction fees in the mempool since the attacker keeps more un-mined transactions in the mempool than the honest miners.
Therefore, if an honest miner mines a block, he gets higher reward and at the same time deposits a higher amount from transaction fees to $\mathcal{FRSC}$s, which indicates a certain self-regulation of our approach, mitigating this kind of attack.

Additionally, we can think of lowering the impact of this attack by rewarding the miner with the full $nextClaim_{[H+1]}$ by $\mathcal{FRSC}$s only if the block contains enough transaction fees (e.g., specified by the network-regulated minimum threshold).
However, this assumes that there is always a reasonable amount of fees in the mempool, which might not be the case all the time and might result in a situation where the miners temporarily stop mining if there is not enough transactions to mine.
Nonetheless, it would require a more research to investigate this solution or a better solution mitigating this type of potential abusive attack, which we left for future work.


%However, this does not seem like a proper solution in case the system would provide higher provisions for honest miners in way of increased transaction fees to be included in a block as mentioned before without the need to complicate $\mathcal{FRSC}$s.

%\subsection{Misusing the Mining Gap}
%\ih{Can be mining gap misused somehow that the adversary can earn more than if she were honest? If not, justify. }
%\is{Probably the same/similar as \mathcal{FRSC}-drying attack. Attacker starts mining when $\mathcal{FRSC}$s are saturated, but there are few txs in mempool, gets reward and stops = attacker gets reward from $\mathcal{FRSC}$s, but contributes back to $\mathcal{FRSC}$s minimally. Can be damaging to the system, but the attacker does not benefit more than if he followed protocol.}

\subsection{Possible Improvements}
$\mathcal{FRSC}$ can contain the parameter enabling the interval of the possible change in the reward paid by $\mathcal{FRSC}^x$ (i.e., $nextClaim_{[H+1]}^{x}$) from the median of its value (computed over $\lambda$).
%
If $nextClaim_{[H+1]}^{x}$ would drastically increase from its median value as significantly more fees would come into the mempool, then $\mathcal{FRSC}_{[H]}^{x}$ would reward the miner with a certain value (specified by the parameter) from the interval $\langle average,nextClaim_{[H+1]}^{x} \rangle$ instead of the full $nextClaim_{[H+1]}^{x}$.
This would be particularly useful for $\mathcal{FRSC}$s with a small $\lambda$ parameter.
The parameter used for sampling might contain a stochastic function (e.g., exponential) attributing a higher likelihood of getting the values not far from the median.
However, we left the evaluation of this technique to future work.

%\textbf{Note:} This functionality is already programmed in the $\mathcal{FRSC}$s but is not propagated into the configuration file and is set to amount, which is not possibly surpassed during our experiments.
%Here you could also specify new $\lambda$, from which we would be calculating $average$.

\subsection{Adjustment of Mining Difficulty}
If the PoW blockchain with the longest chain fork-choice rule uses transaction-fee-based regime, the profitability of miners might be more volatile, which can further lead to decreased security w.r.t. undercutting attacks.
%The end user would also suffer from varying time between blocks.
Although our solution with $\mathcal{FRSC}$s helps in mitigation of this problem, we propose another functionality that resides in adjusting the mining difficulty based on the total collected fees during the epoch.
In detail, the difficulty can be increased with higher fees collected from transactions during the epoch and vice versa.
%This means, that if we calculate profitability solely in native currency and the transaction fees increases during the epoch, we can  partially adjust the difficulty.
Further research would be needed to evaluate this proposition.

%\subsection{Future Work}
%Main goal of this paper was to demonstrate the possible solution for dealing with solely transaction fee-secured protocols.
%Further work would need to be conducted to find perfect balance of individual $\mathcal{FRSC}$s and their parameters.
%This can target different scenarios and different distribution of individual $\mathcal{FRSC}$s, for example as we used exponential distribution for our multiple $\mathcal{FRSC}$s experiment.

==> sec/evaluation.tex <==
We evaluated our proof-of-concept implementation of $\mathcal{FRCS}$s on a long term scenario that we designed to demonstrate significant changes in the total transaction fees in the mempool evolving across the time.
This scenario is depicted in the resulting graphs of most of our experiments, represented by the ``\textit{Fees in mempool}'' series -- see \autoref{sec:exp1} and \autoref{sec:exp2}.
%In experiment, we consider only two miners, where one is legitimate


We experimented with different parameters and investigated how they influenced the total rewards of miners coming from $\mathcal{FRSC}$s versus the baseline without our solution.
Mainly these included a setting of $\mathbb{C}$ as well as different lengths $\lambda$ of $\mathcal{FRSC}$s.
Note that we used the value of transaction fees per block equal to 50 BTC, alike in the original paper introducing undercutting attacks~\cite{carlsten2016instability}.
Also, in all our experiments but the last one (i.e., \autoref{sec:exp4}), we enabled the full mempool option to ensure more realistic conditions.

\begin{figure*}[t]
	\vspace{-0.7cm}
	\centering
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/fees-2016-1-50.png}
			\vspace{-0.9cm}
		\caption{$\mathcal{FRSC}^{1}$ and $\mathbb{C} = 0.5$.}
	\end{subfigure}
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/fees-1-50.png}
					\vspace{-0.9cm}
		\caption{$\mathcal{FRSC}^{2}$ and $\mathbb{C} = 0.5$.}
	\end{subfigure}
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/fees-2016-1-70.png}
					\vspace{-0.9cm}
		\caption{$\mathcal{FRSC}^{1}$ and $\mathbb{C} = 0.7$.}
	\end{subfigure}
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/fees-1-70.png}
					\vspace{-0.9cm}
		\caption{$\mathcal{FRSC}^{2}$ and $\mathbb{C} = 0.7$.}
	\end{subfigure}
	
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/fees-2016-1-90.png}
					\vspace{-0.9cm}
		\caption{$\mathcal{FRSC}^{1}$ and $\mathbb{C} = 0.9$.}
	\end{subfigure}
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/fees-1-90.png}
					\vspace{-0.9cm}
		\caption{$\mathcal{FRSC}^{2}$ and $\mathbb{C} = 0.9$.}
					\vspace{-0.4cm}
	\end{subfigure}
	
	\caption{Experiment I investigating various $\mathbb{C}s$ and $\lambda$s of a single $\mathcal{FRSC}$, where
		$\mathcal{FRSC}^{1}.\lambda = 2016$ and 		$\mathcal{FRSC}^{2}.\lambda = 5600$.
		\textit{Fees in mempool} show the total value of fees in the mined block (i.e., representing the baseline).
		%	This is value a miner would receive if there were no $\mathcal{FRSC}$s.\par
		\textit{Block Value} is the reward a miner received in block $B$ as a sum of the fees he obtained directly (i.e. $\mathbb{M} * B.fees$) and the reward he got from $\mathcal{FRSC}$ (i.e., $nextClaim_{[H]}$).
		\textit{Expected income from Contract} represents the reward of a miner obtained from $\mathcal{FRSC}$ (i.e., $nextClaim_{[H]}$).}\label{fig:50tocontract}
\end{figure*}


\subsection{Experiment I}
\label{sec:exp1}

%\ih{this seems redundant and was mentioned already}
%We will observe both parameters simultaneously as separating them is not a viable option.
%We have created a custom scenario of incoming transaction fees, which is utilized in \autoref{sec:exp1} \& \autoref{sec:exp2} and contains significant changes of transaction fees with jumps in value and later with linearly increasing and decreasing slope.
%This scenario aims to exaggeratedly resemble changes in transaction fees occurring in a real system. \\ \par

\subsubsection{\textbf{Methodology}}
The purpose of this experiment was to investigate the amount of the reward a miner received with our approach versus the baseline (i.e., the full reward is based on all transaction fees).
In this experiment, we investigated how $\mathbb{C}$ influences the total reward of the miner and how $\lambda$ of the sliding window averaged the rewards.
%
In detail, we created two independent $\mathcal{FRSC}$s with different $\lambda$ -- one was set to 2016 (i.e., $\mathcal{FRCS}^1$), and the second one was se to 5600 (i.e., $\mathcal{FRCS}^2$). % respectively.
We simulated these two $\mathcal{FRCS}$s with three different values of $\mathbb{C} \in \{0.5,~0.7,~0.9\}$.

%\begin{center}
%	$\mathcal{FRSC}s^{1} = {\mathcal{FRSC}^{1}(\_, 2016, 1)}$
%	$\mathcal{FRSC}s^{2} = {\mathcal{FRSC}^{1}(\_, 5600, 1)}$
%\end{center}
%
%\textbf{Note} the $value$ is dynamically calculated based on value of $\mathbb{C}$ using \autoref{eq:setup} with $\overline{fees} = 50 BTC$ for the initial setup.

\subsubsection{\textbf{Results}}
The results of this experiment are depicted in \autoref{fig:50tocontract}.
Across all runs of our experiment we can observe that $\mathcal{FRSC}^{2}$ adapts slower as compared to $\mathcal{FRSC}^{1}$, which leads to more significant averaging of the total reward paid to the miner.
Even though this is desired, we can see faster adaptation to changing environment by $\mathcal{FRSC}^{1}$, what a miner can expects from rising fees.
%That is where the \autoref{sec:exp2} comes in, as it keeps the same scenario but with multiple $\mathcal{FRSC}$s better reflects changing environment.



%\iffalse
%\begin{wrapfigure}{r}{0.22\textwidth}
%	\includegraphics[width=0.22\textwidth]{images/fees-legend.png}
%	\ih{this seems wrong - better if you embed the legend into the graphs.}
%\end{wrapfigure}
%\fi




\begin{figure*}
	\vspace{-0.5cm}
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/fees-4-50.png}
		\caption{Scenario with 4 $\mathcal{FRSC}$s,\\ $\mathbb{C} = 0.5$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/contracts-4-50.png}
		\caption{$\partial Claim$s and $nextClaim$, \\ $\mathbb{C} = 0.5$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/normalized-contracts-4-50.png}
		\caption{$\partial Claim$s normalized by $\rho$, \\ $\mathbb{C} = 0.5$.}
	\end{subfigure}

%%%%%%%%%%%%%%%%

	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/fees-4-70.png}
		\caption{Scenario with 4 $\mathcal{FRSC}$s,\\ $\mathbb{C} = 0.7$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/contracts-4-70.png}
		\caption{$\partial Claim$s and $nextClaim$, \\ $\mathbb{C} = 0.7$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/normalized-contracts-4-70.png}
		\caption{$\partial Claim$s normalized by $\rho$, \\ $\mathbb{C} = 0.7$.}
	\end{subfigure}

%%%%%%%%%%%%%%%%

	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/fees-4-90.png}
		\caption{Scenario with 4 $\mathcal{FRSC}$s, \\ $\mathbb{C} = 0.9$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/contracts-4-90.png}
		\caption{$\partial Claim$s and $nextClaim$, \\ $\mathbb{C} = 0.9$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/normalized-contracts-4-90.png}
		\caption{$\partial Claim$s normalized by $\rho$, \\ $\mathbb{C} = 0.9$.}
	\end{subfigure}
	
	\caption{Experiment II investigating various $\mathbb{C}$s in the setting with multiple $\mathcal{FRSC}$s with their corresponding $\lambda$ = $\{1008, 2016, 4032, 8064\}$ and $\rho$ = $\{0.07, 0.14, 0.28, 0.51\}$. $\partial Claim$s represents contributions of individual $\mathcal{FRSC}$s to the total reward of the miner (i.e., its $nextClaim$ component).}\label{fig:exp-II}
\end{figure*}



\begin{figure*}
%	\vspace{-0.5cm}
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/contracts-4-original.png}
		\caption{$\rho$ correlating with $\lambda$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/contracts-4-equal.png}
		\caption{$\rho$ equal for every $\mathcal{FRSC}$.}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{images/contracts-4-inverse.png}
		\caption{$\rho$ negatively correlating with $\lambda$.}
	\end{subfigure}

	\caption{Experiment II -- multiple $\mathcal{FRSC}$s using various distributions of $\rho$ and their impact on $\partial Claim$, where $\mathbb{C}$ = 0.7.}	\label{fig:percentages}
\end{figure*}

\begin{figure}
%	\vspace{-0.3cm}
	\centering
	\begin{subfigure}{0.44\textwidth}
		\includegraphics[width=\textwidth]{images/fees-1-percentage.png}
		\caption{A custom fee scenario for Experiment III.}\label{fig:exp3-fees}
	\end{subfigure}
	\begin{subfigure}{0.44\textwidth}
		\includegraphics[width=\textwidth]{images/percentage.png}
		\caption{A relative difference in $nextClaim$ between 4 $\mathcal{FRSC}$s and a single $\mathcal{FRSC}$.}\label{fig:exp3-relative-diff}
	\end{subfigure}
	
	\caption{Experiment III comparing 4 $\mathcal{FRSC}$s and 1 $\mathcal{FRSC}$, both configurations having the same $\text{effective}\_\lambda$.  }\label{fig:effective_length}
\end{figure}


\subsection{Experiment II}
\label{sec:exp2}

%We will observe how multiple $\mathcal{FRSC}$s deal with the same scenario from \autoref{sec:exp1} and we will look inside individual $\mathcal{FRSC}$s to see their total and normalized values.

\subsubsection{\textbf{Methodology}}
In this experiment, we investigated how multiple $\mathcal{FRSC}$s dealt with the same scenario as before -- i.e., varying $\mathbb{C}$.
In detail, we investigated how individual $\mathcal{FRSC}$s  contributed to the $nextClaim_{[H+1]}$ by their individual $\partial Claim^{\mathcal{FRSC}_{[H]}}_{[H+1]}$.
%
This time, we varied only the parameter $\mathbb{C} \in \{0.5, ~0.7, ~0.9\}$, and we considered four $\mathcal{FRSC}$s:
\begin{center}
	$\mathcal{FRSC}s=\{$\\
	$\mathcal{FRSC}^{1}(\_, 1008, 0.07), \mathcal{FRSC}^{2}(\_, 2016, 0.14),$\\
	$\mathcal{FRSC}^{3}(\_, 4032, 0.28), \mathcal{FRSC}^{4}(\_, 8064, 0.51)\},$
\end{center}
where their lengths $\lambda$ were set to consecutive powers of two (to see differences in more intensive averaging spread across longer intervals), and their redistribution ratios $\rho$ were set to maximize the potential of averaging by longer $\mathcal{FRSC}$s (see details below in \autoref{sec:different-rhos}). 

%However we will show additional data, that is valuable in multi-$\mathcal{FRSC}$ environment.
%The purpose of this experiment is to show, how different $\mathcal{FRSC}$s inside $\mathcal{FRSC}s$ setup are affected and their impact on the final reward going to the miner.\ \\ \par



\subsubsection{\textbf{Results}}
%We have verified the expected advantages of using multi-$\mathcal{FRSC}$ setup.
The results of this experiment are depicted in \autoref{fig:exp-II}.
We can observe that the shorter $\mathcal{FRSC}$s quickly adapted to new changes and the longer $\mathcal{FRSC}$s kept more steady income for the miner.
In this sense, we can see that $\partial Claim^{4}$ held steadily over the scenario while for example $\partial Claim^{1}$ fluctuated more.
%

Since the scenarios of fees evolution in the mempool was the same across all our experiments (but \autoref{sec:exp3}), we can compare the $\mathcal{FRSC}$ with $\lambda$ = 5600 from \autoref{sec:exp1} and the current setup involving four $\mathcal{FRSC}$s -- both had some similarities.
This gave us intuition for replacing multiple $\mathcal{FRSC}$s with a single one, which we further investigated in \autoref{sec:exp3}.

%This was done intentionally to compare, if we are able to interchange multi-$\mathcal{FRSC}$ setup with a single $\mathcal{FRSC}$ using $effective\_\lambda$, which we will introduce in \autoref{sec:exp3}.

\subsubsection{\textbf{Different $\rho$s}}\label{sec:different-rhos}
In \autoref{fig:percentages} we investigated different values of $\rho$ in the same set of four contracts and their impact on $\partial Claim$s.
%We set $\mathbb{C}$ to 0.7 with individual $\mathcal{FRSC}$s' $\rho$s set to different ratios.
The results show that the values of $\rho$ should correlate with $\lambda$ of multiple $\mathcal{FRSC}$s to maximize the potential of averaging by longer $\mathcal{FRSC}$s.


\subsection{Experiment III}\label{sec:exp3}
\subsubsection{\textbf{Methodology}}
In this experiment, we investigated whether it is possible to use a single $\mathcal{FRSC}$ setup to replace a multiple $\mathcal{FRSC}$s while preserving the same effect on the $nextClaim$.
%
To quantify a difference between such cases, we introduced a new metric of $\mathcal{FRSC}s$, called $\text{effective}\_\lambda$, which can be calculated as follows:
\begin{eqnarray} \label{eq:effective_length}	
	\text{effective}\_\lambda (\mathcal{FRSC}s) = \sum_{x ~\in~ \mathcal{FRSC}s} x.\rho* x.\lambda.
\end{eqnarray}
%
As the example, we were interested in comparing a single $\mathcal{FRSC}$ with 4 $\mathcal{FRSC}$s, both configurations having the equal $\text{effective}\_\lambda$. 
The configurations of these two cases are as follow: 
(1) $\mathcal{FRSC}(\_, 5292, 1)$ and (2)
\begin{center}
	$\mathcal{FRSC}s=\{$\\
	$\mathcal{FRSC}^{1}(\_, 1008, 0.07), \mathcal{FRSC}^{2}(\_, 2016, 0.19),$\\
	$ \mathcal{FRSC}^{3}(\_, 4032, 0.28), \mathcal{FRSC}^{4}(\_, 8064, 0.46)\}$.
\end{center}
%
We can easily verify that the $\text{effective}\_\lambda$ of 4 $\mathcal{FRSC}$s is the same as in a single $\mathcal{FRSC}$ using \autoref{eq:effective_length}:
$0.07 * 1008 + 0.19 * 2016 + 0.28 * 4032 + 0.46 * 8064 = 5292$.



We conducted this experiment using a custom fee evolution scenario involving mainly linearly increasing/decreasing fees in the mempool (see \autoref{fig:exp3-fees}), and we set $\mathbb{C}$ to 0.7 for both configurations.
The new scenario of the fee evolution in mempool was chosen to contain extreme changes in fees, emphasizing possible differences.


\subsubsection{\textbf{Results}}
In \autoref{fig:exp3-relative-diff}, we show the relative difference in percentages of $nextClaim$ rewards between the settings of 4 $\mathcal{FRSC}$s versus 1 $\mathcal{FRSC}$.
%
It is clear that the setting of 4 $\mathcal{FRSC}$s  in contrast to a single $\mathcal{FRSC}$ provided better reward compensation in times of very low fees value in the mempool, while it provided smaller reward in the times of higher values of fees in the mempool.
%
Therefore, we concluded that it is not possible to replace a setup of multiple $\mathcal{FRSC}$s with a single one. % even though in more realistic environment we might see much smaller differences due to 
%
%We can better observe this from the results of continuous linear changes in fees.
%That is why this extreme case was used. 
%However, in environment with milder extremes we might see less significant differences. % as if we compare the corresponding graphs from \autoref{sec:exp1} and \autoref{sec:exp2}.

\subsection{Experiment IV}\label{sec:exp4}
We focused on reproducing the experiment from Section 5.5 of~\cite{carlsten2016instability}. % found under figure 6 with our $\mathcal{FRSC}$-based solution.
We were searching for the minimal ratio of \textsc{Default-Compliant} miners, at which the undercutting attack is no longer profitable strategy.
\textsc{Default-Compliant} miners are honest miners in a way that they follow the rules of the consensus protocol such as building on top of the longest chain.
% and not trying to intentionally fork the chain.
%In case we have two chains \textsc{Default-Compliant} miner mines on the older chain.

We executed several simulations, each consisting of multiple games (i.e., 300k as in~\cite{carlsten2016instability}) with various fractions of \textsc{Default-Compliant} miners.
From the remaining miners we evenly created \textit{learning miners}, who learn on the previous runs of games and switch with a certain probability the best mining strategy out of the following.
%\is{??? meaning?}
\begin{compactitem}
	\item \textsc{PettyCompliant}: This miner behaves as \textsc{Default-Compliant} except one difference.
	In the case of seeing two chains, he does not mine on the oldest block but rather the most profitable block.
	Thus, this miner is not the (directly) attacking miner.

	\item \textsc{LazyFork}:
	This miner checks which out of two options is more profitable: (1) mining on the longest-chain block or (2) undercutting that block.
	In either way, he leaves half of the mempool fees for the next miners, which prevents another \textsc{LazyFork} miner to undercut him.
	
	\item \textsc{Function-Fork()}
	The behavior of the miner can parametrized with a function f(.) expressing the level of his undercutting.
	The higher the output number the less reward he receives and more he leaves to incentivize other miners to mine on top of his block.
	This miner undercuts every time he forks the chain. % and he has to undercut with his function f(.) parameter.	
\end{compactitem}
	




\subsubsection{\textbf{Methodology}}
With the missing feature for difficulty re-adjustment  (present in our work as well as in~\cite{carlsten2016instability}) the higher orphan rate occurs, which might directly impact our $\mathcal{FRSC}$-based approach.
If the orphan rate is around 40\%, roughly corresponding to~\cite{carlsten2016instability}, our blocks would take on average 40\% longer to be created, increasing the block creation time (i.e., time to mine a block).
%With that the mean blocktime differs from what we expect.
This does not affect the original simulator, as there are no $\mathcal{FRSC}s$ that would change the total reward for the miner who found the block.

%To extrapolate the final value, i.e., sum of all rewards of miners of all the transaction fees, in the longest chain is:
%\begin{center}
%	$(head().timestamp - genesis().timestamp) * feeRate$,
%\end{center}
%where the $feeRate$ corresponds to constant fees incoming every second into the mempool (as in the original simulator), $head()$ returns the highest block from the longest chain, and	$genesis()$ returns the genesis block.



Nevertheless, this is not true for $\mathcal{FRSC}$-based simulations as the initial setup of $\mathcal{FRSC}s$ is calculated with $\overline{fees} = 50$ BTC (as per the original simulations).
However, with longer block creation time and transaction fees being calculated from it, the amount of $\overline{fees}$ also changes.
Without any adjustments this results in $\mathcal{FRSC}s$ initially paying smaller reward back to the miner before they are saturated. % themselves enough.
To mitigate this problem, we increased the initial values of individual $\mathcal{FRSC}$s by the orphan rate from the previous game before each run.
This results in very similar conditions, which can be verified  by comparing the final value in the longest chain of our simulation versus the original simulations.
We decided to use this approach to be as close as possible to the original experiment.
This is particularly important when the parameter for the full mempool is equal to $false$ (see \autoref{sec:implementation}), which means that the incoming transaction fees to mempool are calculated based on the block creation time. 
%\is{what does mempool parameter does? what does true/false actually mean?}\par
In our simulations, we used the following parameters: 100 miners,
	10 000 blocks per game, %\is{define game, run of the simulation?}
	300 000 games (in each simulation run),
	exp3 learning model, and
	$\mathbb{C} = 0.7$.
Modeling of fees utilized the same parameters as in the original paper~\cite{carlsten2016instability}: the full mempool parameter disabled, a constant inflow of 5 000 000 000 Satoshi (i.e., 50 BTC) every 600s.
For more details about the learning strategies and other parameters, we refer the reader to~\cite{carlsten2016instability}.

\subsubsection*{\textbf{Setup of $\mathcal{FRSC}s$}}
Since we have a steady inflow of fees to the mempool, we do not need to average the income for the miner.
Therefore, we used only a single $\mathcal{FRSC}$ defined as $\mathcal{FRSC}$(7 056 000 000 000, 2016, 1), where the initial value of $\mathcal{FRSC}.\nu$ was adjusted according to \autoref{eq:setup}, assuming $\overline{fees} = 50$ BTC.
%
In next runs of any game, $\mathcal{FRSC}.\nu$ was increased by the orphan rate from the previous runs, as mentioned above.

\begin{figure}
%	\vspace{-0.5cm}
	\centering
	\begin{subfigure}{0.40\textwidth}
		\includegraphics[width=\textwidth]{images/equilibrium.png}
	\end{subfigure}
	
\caption{The number of \textsc{Default-Compliant}  miners in our $\mathcal{FRSC}$ approach is $\sim$30\% (in contrast to $\sim66\%$ of~\cite{carlsten2016instability}).}\label{fig:improvement}
\end{figure}

%\textbf{Note 2.} For more details about the learning strategies, how the simulations are conducted and full list of other parameters please navigate to the original paper \cite{carlsten2016instability}.\\

\subsubsection{\textbf{Results}}
The results of this experiment are depicted in \autoref{fig:improvement}, and they demonstrate that with our approach using $\mathcal{FRSC}$s, we lowered down the number of \textsc{Default-Compliant} miners (i.e., purple meeting red) from the original $66\%$ to $30\%$.
This means that the profitability of undercutting miners is avoided with at least $30\%$ of \textsc{Default-Compliant} miners, indicating the more robust results. 
%\ih{How different values of $\mathbb{C}$ impact the results?}

%This implies more robust system against undercutting attacks, which were presented in the paper~\cite{carlsten2016instability}.
%

==> sec/implementation.tex <==
Our implementation is based on Bitcoin Mining Simulator~\cite{bitcoin_mining_simulator:kalodner}, introduced in~\cite{carlsten2016instability}, which was adjusted to our needs.

\subsubsection{Changes in Simulator}
%Compared to the original scenario of linearly incoming transaction fees we have decided to create configuration file %\footnote{Called feeSimulation.json}
%to simulate custom scenarios of incoming transactions.
%We have reconfigured the fixed behavior of fees linearly incoming to mempool described in Section 3.2 of~\cite{carlsten2016instability} to optional with the parameter enabling to switch simulation into the mode with the full mempool.
%\footnote{fullMempool parameter in feeSimulation.json}. \ih{Too detailed for the paper.}
%This option is important to use, as with forking attacks the chain does not adjust itself to adopt the slower rate of blocks as it does not support this possibility.
%This results in more difficult initial setup of contracts and we argue this simulation of fees better represents real conditions~\cite{b2,b3}\\  \par

We have created a configuration file to simulate custom scenarios of incoming transactions instead of the original design~\cite{carlsten2016instability} fees.
We added an option to switch simulation into a mode with a full mempool, and thus bound the total fees (and consequently the total number of transactions) that can be earned within a block -- 
this mostly relates to blocks whose mining takes longer time than the average time to mine a block.\footnote{Note that the original simulator~\cite{carlsten2016instability} assumes that the number of transactions (and thus the total fees) in the block is constrained only by the duration of a time required to mine the block, which was also criticized in~\cite{gong2022towards}.}
%This option is essential when simulating forking attacks, as the chain is unprepared for this possibility and therefore does not adapt to the slower rate of blocks.
%This option should be more representative of stable utilization of blockchain in the future.
%It also allows us to clearly evaluate our simulation results.
%With this reconfiguration of the simulator, the initial setup of our contracts is more straightforward and sufficiently represents real-world conditions.

%To make running the simulator easier without the need to reconfigure and recompile the program we have moved some parameters as start-up arguments of the program.
%Finally we have integrated our proposed contract-based solution into the simulator.
%These contracts are also able to be set-up by corresponding configuration file. %\footnote{feeContracts.json}.
%All our testing was done with values corresponding to the original simulator, i.e. the base value of transaction fees per block is 50BTC.

Next, we moved several parameters to arguments of the simulator with the intention to eliminate the need of recompilation the program frequently, and therefore simplify the process of running various experiments with the simulator.
Finally, we integrated our $\mathcal{FRCS}$-based solution into the simulator.
$\mathcal{FRSC}$s are initiated from a corresponding configuration file.
The source code of our modified simulator is available at anonymous link \url{https://www.dropbox.com/s/gwlbedq47csthqp/sources.zip?dl=0}.


==> sec/introduction.tex <==
% Not proper for problem definition, possible inspiration for introduction
Cryptocurrencies provide block rewards to incentivize miners in producing new blocks.
Transaction fees also contribute to the revenue of miners, motivating them to include transactions in blocks.
Miners maximize their profits by prioritizing the transactions with the highest fees.
%On top of block rewards, miners are incentivized by transaction fees to include transactions in the blocks, while they try to maximize their profit as the sum of the block reward and the most abundant transactions selected into the block. 
In Bitcoin and its numerous clones~\cite{hum2020coinwatch}, the block reward is divided by two approx. every four years (i.e., after every 210k blocks), which will eventually result in a pure transaction-fee-based regime.

Before 2016, there was a belief that the dominant source of the miners' income does not impact the security of the blockchain.
%However, Carlsten et al.~\cite{carlsten2016instability} showed that it is not the case, while they pointed out that with transaction-fee-based regime, the variance of the block reward is very high due to the exponentially distributed block arrival time, which makes attractive to fork a wealthy block and thus steal the transaction fees.
However, Carlsten et al.~\cite{carlsten2016instability} pointed out the effects of the high variance of the miners' revenue per block caused by exponentially distributed block arrival time in transaction-fee-based protocols.
The authors showed that \emph{undercutting} (i.e., forking) a wealthy block is a profitable strategy for a malicious miner. % in transaction-fee-based regimes of blockchain.
Nevertheless, Daian et al.~\cite{daian2020flash} showed that this attack is viable even in blockchains containing traditional block rewards due to front-running competition of arbitrage bots who are willing to extremely increase transaction fees to earn Maximum Extractable Value profits.
 % which might on top of it involve double spending attacks.

%Since the creation of Bitcoin many pointed out possible problems with such blockchains living purely from their transaction fees.\ih{put 1-2 citations on those who claimed it. Maybe it would be nice to briefly hear what problems do you mean here.}
%Not much thought was given to this problem in the Bitcoin whitepaper~\cite{nakamoto2008bitcoin}, citing the author, \say{\textit{Once a predetermined number of coins have entered circulation, the incentive can transition entirely to transaction fees and be completely inflation free.}}\par

%In this paper, we will focus on transaction-fee-based regime of Proof-of-Work blockchains, and we empirically evaluate a mitigation technique for the ``forking wealthy block'' problems described in~\cite{carlsten2016instability} as well as other problems that might exist (not only) in transaction fee based regime.
%In particular, we focus on improving initial profits of new miners (i.e., the mining gap) enabling to cover their expenses and the problem of transaction fees fluctuation what impact the reward variance of miners.
In this paper, we focus on mitigation of the undercutting attack in transaction-fee-based regime of PoW blockchains.
We also discuss related problems present (not only) in transaction-fee-based regime.
In particular, we focus on minimizing the mining gap~\cite{carlsten2016instability,tsabary2018gap}, (i.e., the situation, where the immediate reward from transaction fees does not cover miners' expenditures) as well as balancing significant fluctuations in miners' revenue.

%To deal with these problems, we propose a solution that aggregates a certain part of transaction fees from mined blocks in one or more smart contracts, while at the same time it enables the redemption from these smart contracts.
%This setting enables us to achieve several interesting properties that are beneficial for the consensus protocol.

To mitigate these issues, we propose a solution that splits  transaction fees from a mined block into two parts -- (1) an instant reward for the miner and (2) a deposit sent into one or more fee-redistribution smart contracts ($\mathcal{FRSC}$s).
At the same time, these $\mathcal{FRSC}$s reward the miner of a block with a certain fraction of the accumulated funds over a fixed period of time (i.e., the fixed number of blocks).
This setting enables us to achieve several interesting properties that are beneficial for the stability and security of the protocol.

\subsubsection*{\textbf{Contributions}}
In detail, our contributions are as follows:
\begin{enumerate}
	\item We propose an approach that normalizes the mining rewards coming from transaction fees by one or more $\mathcal{FRSC}$s that perform moving average on a certain portion of the transaction fees.
	
	\item We evaluate our approach using various fractions of the transaction fees from a block distributed between a miner and $\mathcal{FRSC}$s.
	We experiment with the various numbers and lengths of $\mathcal{FRSC}$s, and we demonstrate that usage of multiple $\mathcal{FRSC}$s of various lengths has the best advantages mitigating the problems we are addressing; however, even using a single $\mathcal{FRSC}$ is beneficial.
	
%	We found out that \ih{1) the best value was ... 2) especially in a combination with multiple contracts .... }
	
	\item We demonstrated that with our approach, the mining gap can be minimized since the miners at the beginning of the mining round can get the reward from $\mathcal{FRSC}$s, which stabilizes their income.
	
	\item We empirically demonstrate that using our approach the threshold of \textsc{Default-Compliant} miners who strictly do not execute undercutting attack is lowered from 66\% (as reported in the original work~\cite{carlsten2016instability}) to 30\%. 
%	\ih{Does it make sense to mention 51\% of honest portion of PoW? I think it does not relate, but think of it.}
	
\end{enumerate}

%\subsubsection*{\textbf{Organization}}
%This paper is organized as follows. 
%\autoref{sec:problemdefinition} defines the problem that we are dealing with.
%In \autoref{sec:proposedapproach}, we describe our approach.
%In \autoref{sec:evaluation},  we conduct the experiments to evaluate our approach in terms of lowering the profitability of undercutting attacks.
%\ih{TODO last}

%During this paper we will use Bitcoin's BTC currency. This should be noted somewhere

==> sec/problemdefinition.tex <==
In transaction fee-based regime schemes, a few problems have emerged, which we can observe even nowadays in Bitcoin protocol~\cite{carlsten2016instability}.
We have selected three main problems and aim to lower their impact for protocols relying only on transaction fees. 
%without additional inflation to incentivize miners.\par
In detail, we focus on the following problems:


\begin{enumerate}
	\item \textbf{Undercutting attack.}
	%directly causing higher orphan rate and unreliable functionality of the system.
	%To summarize the root cause of the problem:\par
	%Consider new transactions entering mempool with reasonably high feeRates~\cite{b5}.\footnote{As described on the website, the total fee divided by the size of transaction.}
	In this attack, a malicious miner attempts to obtain transaction fees by re-mining a top block of the longest chain, and thus motivates other miners to mine on top of her block~\cite{carlsten2016instability}.
	%
	In detail, consider a situation, where an honest miner mines a block containing transaction with extremely high transaction fees. % in contrast to common transaction fees.
	The malicious miner can fork this block while he leaves some portion of the ``generous'' transactions un-mined in the mempool.
	These transactions motivate other miners to mine on top of the attacker's chain, and thus undercut the original block. % as it would yield him a higher reward, then mining on top of the original block.
	Such a malicious behavior might result in higher orphan rate, unreliability of the system, and double spending.
	%
%	This problem is investigated in~\cite{carlsten2016instability}.
%	\is{defining feeRate is not necesary for the explanation of this attack, define if needed later in the paper}
	
	\item \textbf{The mining gap.}
	As discussed in~\cite{carlsten2016instability}, the problem of mining gap arises once the mempool does not contain enough transaction fees to motivate miners in mining.
	Suppose a miner succeeds at mining a new block shortly after the previous block was created, which can happen due to well known exponential distribution of block creation time in PoW blockchains.
	Therefore, the miner might not receive enough rewards to cover his expenses because most of the transactions from the mempool were included in the previous block, while new transactions might not have yet arrived or have small fees.
	Consequently, the miners are motivated to postpone mining until the mempool is reasonably filled with enough transactions (and their fees).
	The mining gap was also analyzed by the simulation approach in the work of Tsabary and Eyal~\cite{tsabary2018gap}, who further demonstrated that this mining gap incentivizes larger mining coalitions, which impacts decentralization.
	%is also described in the paper~\cite{carlsten2016instability} from previous point. The problem lies if miner decides to not mine if there is not enough in transaction fee rewards in the mempool to cover his operational costs.
	%Meaning if a miner starts mining fresh block with little value in the mempool, as most of the transaction were included in the previous block, and successfully mines such block he would not receive enough reward to cover his expenses.
	%That is the reason for him to not mine until the mempool is reasonable filled with transactions.
	
	\item \textbf{Varying transaction fees over time.}
	%can cause higher fluctuation of miner's revenue during certain time frames, e.g. even over a span of day or week~\cite{b5}.
	In the transaction-fee-based regime, any fluctuation in transaction fees directly affects the miners' revenue.
	High fluctuation of transaction fees during certain time frames, e.g., in a span of a day or a week~\cite{b5}, can lead to an undesirable lack of predictability in rewards of miners and indirectly affect the security of the underlying protocol.
	
	%We can expect a similar behavior during times of holidays \ih{why? I'd drop this claim.}.
	%This phenomenon can make chain prone to instability in profitability of miners, indirectly effecting security of the underlying protocol.
	
\end{enumerate}





%\subsection{Overview}
%\ih{This section seems useless since we already have overview in the next section. I'd drop it. Picture is ok.}


==> sec/proposedapproach.tex <==
%We propose to integrate simple redistribution contract(s) into the blockchain protocol.
%This contract would collect fraction of fees from mined transactions, while averaging and paying these fees back to the miners.

%Our proposed solution would lead to averaging the rewards of fees in case of fluctuation and also result in more predictable and consistent rewards for the miners.
%With experiments conducted in section \autoref{sec:evaluation} we will see this approach also results in decreased effect of undercutting attacks.
%We will describe the mechanism into more depth and formal definitions under next section \hyperref[proposed approach]{Proposed approach} \ih{use autoref, instead of hyperref}.

In this section, we describe our proposed solution in more detail.
%
\begin{figure}[t]
	\includegraphics[width=0.45\textwidth]{images/explanation.png}
			\vspace{-0.7cm}
	\caption{Overview of our solution. }
%				\vspace{-0.5cm}
	\label{fig:overview}
\end{figure}
%\subsection{Overview}
Our proposed solution collects a percentage of transaction fees in a native cryptocurrency from the mined blocks into one or multiple fee-redistribution smart contracts (i.e., $\mathcal{FRSC}$s).
Miners of the blocks who must contribute to these contracts are at the same time rewarded from them, while the received reward approximates a moving average of the incoming transaction fees across the fixed sliding window of the blocks.
The fraction of transaction fees (i.e., $\mathbb{C}$) from the mined block is sent to $\mathcal{FRSC}$ and the remaining fraction of transaction fees (i.e., $\mathbb{M}$) is directly assigned to the miner, such that $ \mathbb{C} + \mathbb{M} = 1.$

The role of $\mathbb{M}$ is to incentivize the miners in prioritization of the transactions with the higher fees while the role of $\mathbb{C}$ is to mitigate the problems of undercutting attacks and the mining gap.

\medskip\noindent
\subsubsection*{\textbf{Overview}}
We depict the overview of our approach in \autoref{fig:overview}, and it consists of the following steps:
\begin{enumerate}
	
	\item Using $\mathcal{FRSC}$, the miner calculates the reward for the next block $B$ (i.e., $nextClaim(\mathcal{FRSC})$ -- see \autoref{eq:nextClaim}) that will be payed by $\mathcal{FRSC}$ to the miner of that block.
	
	\item The miner mines the block $B$ using the selected set of the highest fee transactions from her mempool.
	
	\item The mined block $B$ directly awards a certain fraction of the transaction fees (i.e., $B.fees ~*~ \mathbb{M}$) to the miner and the remaining part (i.e., $B.fees ~*~ \mathbb{C}$) to $\mathcal{FRSC}$.
	
	\item The miner obtains $nextClaim$ from $\mathcal{FRSC}$.
	
\end{enumerate}
%
Our approach is embedded into the consensus protocol, and therefore consensus nodes are obliged to respect it in order to ensure that their blocks are valid.
It can be implemented with standard smart contracts of the blockchain platform or within the native code of the consensus protocol.





\subsection{Prioritization of High-Fee Transactions}
In the environment with constant transaction fees, a miner would receive the same amount with or without our solution.
However, in public blockchains (especially with transaction-fee based regime) there exist a mechanism to ensure prioritizaiton in processing of transactions with higher fees, which might result into fluctuations in rewards of the miners.
In our approach, we preserve the transaction prioritization since we directly attribute a part of the transaction fees to the miner (i.e., $\mathbb{M}$).


%\ih{Therefore, the purpose of our solution is to cope with the cases of transaction fees fluctuations and ensure more predictable and consistent income for the miners. [drop?]}



%The protocol requires a miner of a block to collect a fraction of the transaction fees into $\mathcal{FRSC}$, and the same time she receives a reward from $\mathcal{FRSC}$.


%Therefore, this mechanism acts as an approximation of ``the base block reward,'' which should ensure that miners have stable income by  




%$\mathbb{M}$ represents the portion of transaction fees a miner keeps from transactions included in a block and $\mathbb{C}$ represents the portion of transaction fees deposited into the redistribution contract.\\ \ih{already mentioned}

\subsection{Fee-Redistribution Smart Contracts}\label{sub:redistrib}
We define the fee-redistribution smart contract as 
\begin{eqnarray}
\mathcal{FRSC} = (\nu, \lambda, \rho), 
\end{eqnarray}
where
$\nu$ is the accumulated amount of tokens in the contract, $\lambda$ denotes the size of $\mathcal{FRSC}$' sliding window in terms of the number of preceding blocks that contributed to $\nu$,
%\footnote{In reality it works as moving average into infinity in case we do not add BTC to the contract}, and
and $\rho$ is the parameter defining the ratio for redistribution of incoming transaction fees among multiple contracts, while the sum of $\rho$ across all $\mathcal{FRSC}$s must be equal to 1:
\begin{eqnarray}\label{eq:frsc-redistrib-ratios}
	\sum_{x ~\in~ \mathcal{FRSC}s} x.\rho &=& 1.
\end{eqnarray}
%
In contrast to a single $\mathcal{FRSC}$, multiple $\mathcal{FRSC}$s enable better adjustment of compensation to miners during periods of higher transaction fee fluctuations or in an unpredictable environment (we show this in \autoref{sec:exp3}).
%Therefore, we require variable $\rho$ of $\mathcal{FRSC}$ to define the redistribution ratio among the individual $\mathcal{FRSC}$s. \ih{redundant - was already mentioned}
%However, this ratio does not directly correspond to the $\mathcal{FRSC} = (\nu, \lambda, \rho)$, 's contribution to the total reward for the miner. \ih{irelevant}

%When using multiple redistribution contracts, we define these as a set of individual contracts, where the following holds: \ih{does not bring more info than was already said}
%\begin{multline} \label{eq:1}
%	\mathcal{FRSC}s = \{contract(\nu, \lambda, \rho)\ | \  \lambda,\rho > 0\ \land \ \nu >= 0\ \land\\
%	\sum_{c\ \in\ \mathcal{FRSC}s}^{}c.\rho = 1	\}
%\end{multline}
%\par

\medskip
We denote the state of $\mathcal{FRSC}$s at the blockchain height $H$ as $\mathcal{FRSC}_{[H]}$.
%We also consider the next block, build on a chain of height $H$ with $\mathcal{FRSC}^{[H]}$, as a block with height $H+1$, where $h = H + 1$. \ih{Intuitive}
%
Then, we determine the reward from $\mathcal{FRSC}_{[H]} \in \mathcal{FRSC}s_{[H]}$ for the miner of the next block with height $H+1$ as follows:
%
\begin{equation}
	\partial Claim_{[H+1]}^{\mathcal{FRSC}_{[H]}} = \frac{\mathcal{FRSC}_{[H]}.\nu}{\mathcal{FRSC}_{[H]}.\lambda},
\end{equation}
while the reward obtained from all $\mathcal{FRSC}$s is
%
\begin{equation} \label{eq:nextClaim}	
nextClaim_{[H+1]} = \sum_{\mathcal{X}_{[H]} ~\in~ \mathcal{FRSC}s_{[H]}^{}} \partial Claim_{[H+1]}^{\mathcal{X}_{[H]}}.
\end{equation}

%Notice that $nextClaim$ is parametrized by $H+1$ as we calculate the reward for the next block of height $h = H + 1$ from the contract balances at height $H$.

\noindent
%This $nextClaim_{[H+1]}$ represents the value of tokens obtained by the miner of the next block with height $H+1$. \ih{already mentioned}
Then, the total reward of the miner who mined the block $B_{[H+1]}$ with all transaction fees $B_{[H+1]}.fees$ is
\begin{equation} \label{eq:rewardtotal}
	rewardT_{[H+1]} = nextClaim_{[H+1]} + \mathbb{M} * B_{[H+1]}.fees.
\end{equation}
%
The new state of contracts at the height $H + 1$ is 
\begin{eqnarray}
	\mathcal{FRSC}s_{[H+1]} = \{\mathcal{X}_{[H+1]}(\nu, \lambda, \rho)\ ~|~
\end{eqnarray}
\begin{eqnarray}
	\lambda &=& \mathcal{X}_{[H]}.\lambda,\\
	\rho &=& \mathcal{X}_{[H]}.\rho,\\
	\nu &=& \mathcal{X}_{[H]}.\nu - \partial Claim_{[H+1]} +  deposit * \rho,\\
	deposit &=& B_{[H+1]}.fees * \mathbb{C}\},
\end{eqnarray}
where $deposit$ represents the fraction $\mathbb{C}$ of all transaction fees from the block $B_{[H+1]}$ that are deposited across all $\mathcal{FRSC}$s in ratios respecting \autoref{eq:frsc-redistrib-ratios}.

\subsection{Example}
%\ih{use Bitocin only in this example; in the whole work use just the blockchain instead, while at the beginning of the paper (intro) we can say that we focus on PoW blockchains in this work, but the results might be applicable also in the setting of PoS.}
We present an example using Bitcoin~\cite{nakamoto2008bitcoin} to demonstrate our approach.
We assume that the current height of the blockchain is $H$, and we utilize only a single $\mathcal{FRSC}$ with the following parameters:
\[
\mathcal{FRSC}_{[H]} = (2016, 2016, 1).
\]
%where $\nu$ of the contract equals to 2016 BTC, redistribution $\lambda$ is targeted for 2016 blocks, i.e. one Bitcoin epoch.
%$\rho$ is currently omitted but it must hold true with the afford-mentioned rule in \autoref{eq:1}.
%Current blockchain height is $H$.
We set $\mathbb{M} = 0.4$ and $\mathbb{C} = 0.6$, which means a miner directly obtains 40\% of the $B_{[H+1]}.fees$ and $\mathcal{FRSC}$ obtains remaining 60\%.



\medskip
\noindent
Next, we compute the reward from $\mathcal{FRSC}$ obtained by the miner of the block with height $H+1$ as 
\begin{equation*}
	\partial Claim_{[H+1]} = \frac{\mathcal{FRSC}_{[H]}.\nu}{\mathcal{FRSC}_{[H]}.\lambda} = \frac{2016}{2016} = 1~\text{BTC},
\end{equation*}
resulting into 
\begin{equation*}
nextClaim_{[H+1]} = \partial Claim_{[H+1]}~=~1~\text{BTC}.
\end{equation*}

%
%\is{The following should not be part of example, but general definition of the approach:}
%We will also notate with $H$ that this state of $contract$ with it's parameters holds true for height $H$.
%Allow us to mark next block, build on chain of height $H$ with our defined $contract$., as block with height $H+1$ which equals to $h = H + 1$.
%We can then calculate the reward from a contract $c \in \mathcal{FRSC}s_{[H]}$ for the next mined block with general formula as follows:
%
%\begin{equation}
%	\partial Claim_{[H+1]}^{c} = \frac{c.\nu}{c.\lambda},
%\end{equation}
%
%while the total reward obtained from all contracts is:
%
%\begin{equation} \label{eq:nextClaim}	nextClaim_{[H+1]} = \sum_{x \in \mathcal{FRSC}s_{[H]}^{}} \partial Claim_{[H+1]}^{x}.
%\end{equation}
%
%Notice that $nextClaim$ is annotated \ih{not annotated but denoted with. but in this case maybe parametrized by.} with $H+1$ as we calculate the reward for the next block of height $h = H + 1$ from the contract balances at height $H$\\
%
%\is{Example continues here:}
%In this example, formula unwraps into the following:
%
%\[
%nextClaim_{[H+1]} = \frac{\mathcal{FRSC}_{[H]}.\nu}{\mathcal{FRSC}_{[H]}.\lambda} = \frac{2016}{2016},
%\]
%which would in our case yield $nextClaim_{[H+1]}   = 1$ BTC.
%This $nextClaim_{[H+1]}$ would be claimable by the miner, who successfully mines the next block of height $H+1$ on top of our chain of height $H$.\par
%
%\medskip
%\subsubsection{\textbf{Forks}}
%We do not consider possible forks on the chain.\\
%To incentivize the miner to prioritize the transactions with the highest fees in the block he mines, 
%\medskip\noindent

\noindent
Further, we assume that the total reward collected from transactions in the block with height $H+1$ is $B_{[H+1]}.fees = 2$ BTC.
Hence, the total reward obtained by the miner of the block $B_{[H+1]}$ is
\begin{eqnarray*}
	rewardT_{[H+1]} &=& nextClaim_{[H+1]}  + \mathbb{M} * B_{[H+1]}.fees \\
	&=& 1 + 0.4 * 2 \\
	&=& 1.8 ~\text{BTC},
\end{eqnarray*}
and the contribution of transaction fees from $B_{[H+1]}$ to the $\mathcal{FRSC}$ is 
\[
deposit = B_{[H+1]}.fees * \mathbb{C} = 1.2 ~\text{BTC}.
\]
Therefore, the value of $\nu$ in $\mathcal{FRSC}$ is updated at height H~+~1 as follows:
\begin{eqnarray*}
	v_{[H+1]} &=& \mathcal{FRSC}_{[H]}.\nu - nextClaim_{[H+1]} + deposit \\
	&=& 2016 - 1 + 1.2  ~\text{BTC} \\
	&=& 2016.2 ~\text{BTC}.
\end{eqnarray*}


% \ih{we do not construct}
%Finally, we construct the set $\mathcal{FRSC}s_{[H+1]}$ with the new state of $\mathcal{FRSC}_{[H+1]}$:
%\[
%\mathcal{FRSC}s_{[H+1]} = \{\mathcal{FRSC}_{[H+1]}(v_{[H+1]}, 2016, 1)\}
%\]


%\ih{This is just a summary}
%Therefore, the state of blockchain at height $H$ was:
%\begin{itemize}
%	\item $\mathcal{FRSC}s_{[H]} = \{\mathcal{FRSC}_{[H]}(2016, 2016, 1)\}$,
%	\item $B_{[H+1]}.fees = 2 \text{ BTC}$,%\footnote{sum of fees in mempool right before block $H+1$ being mined \ih{footnotes should be full sentences.}}\\
%\end{itemize}
%and changes at height $H+1$ ($h = H + 1$) to:
%\begin{itemize}
%	\item $\mathcal{FRSC}s_{[H+1]} = \{\mathcal{FRSC}_{[H+1]}(2016.2, 2016, 1)\}$,
%	\item $rewardT_{[H+1]} = 1.8 \text{ BTC}$.
%\end{itemize}
%

\noindent
\subsubsection*{\textbf{Traditional Way in Tx-Fee Regime}}
In traditional systems (running in transaction-fee regime) $rewardT_{[H+1]}$ would be equal to the sum of all transaction fees $B_{[H+1]}.fees$ (i.e., $2$ BTC); hence, using $\mathbb{M} = 1$. 
%which is higher that the expected mean value of $rewardT_{[H+1]}$, defined as follow:
%\begin{eqnarray}
%	\overline{rewardT_{[H+1]}} &=& 	\frac{nextClaim_{[H+1]}}{\mathbb{C}}.
%\end{eqnarray}  
%We designed our contracts to average $block.fees$ value, in this case to 1.66 BTC.
In our approach, $rewardT_{[H+1]}$ can only be equal to the sum of all transaction fees in the block $B_{[H+1]}$, if:
%In our example this can be simply derived from $\mathbb{C}$ and $nextClaim_{[H+1]}$ as follows:
%\ih{put the name of the variable = .... and period at the end of the sentence, even though it is the formula.}
\begin{eqnarray}
	B_{[H+1]}.fees = \frac{nextClaim_{[H+1]}}{\mathbb{C}}.
\end{eqnarray}
In our example, a miner can mine the block $B_{[H+1]}$ while obtaining the same total reward as the sum of all transaction fees in the block if the transactions carry 1.66 BTC in fees:
\begin{equation*}
B_{[H+1]}.fees = \frac{1}{0.6} = 1.66 ~\text{BTC}.
\end{equation*}




%However this is by design and in the next section we will show how our design should make mining only on transaction fees more predictable and sustainable.

%In the following sections \is{add autoref where, evalutation or discussion?}, we show how our solution contributes to better predictability and sustainability of transaction-fee-based protocols. \ih{ irelevant here.}

%\subsection{Multiple contracts}
%\is{I'd drop this subsection. As I understand it, this is a part of the implementation, not really important for the whole concept. Or maybe move some of it to the section, where multiple contract are first mentioned.}
%%We mentioned the possibility of using multiple contracts.
%%This allows for better adjustment of compensation to miners for sudden changes in rather \ih{unpredictable?} predictable real world environment.
%%For this we introduced variable $\rho$ under tuple $contract$ which states, how much this contract takes from all the fees sent to contracts.
%%However it does not directly correspond to how much value will this contract contribute in calculating $nextClaim$.\\ \par
%With the following formula we create new $\mathcal{FRSC}s_{[H]}$ for height $H$ with newly mined block $B_{[H]}$.\par
%\textbf{Note} the condition from \autoref{eq:1} has to hold, which does not allow us to forget recreation of any contract.
%
%\begin{flushleft}
%	$\mathcal{FRSC}s_{[H]} = \{\mathcal{FRSC}_{[H]}^{x}(\nu, lambda, \rho)\ |$\\
%\end{flushleft}
%\begin{flushright}
%	$back = B_{[H]}.fees * \mathbb{C}\ \land$\\
%	$\mathcal{FRSC}_{H-1}^x \in \mathcal{FRSC}s_{H-1}\ \land$\\
%	$l = \mathcal{FRSC}_{H-1}^{x}\ \land$\\
%	$ \rho = \mathcal{FRSC}_{H-1}^{x}\ \land$\\
%	$v = \mathcal{FRSC}_{H-1}^{x}.\nu - nextClaim_{[H]}^{x} +  back* p\}$\\
%\end{flushright}

\subsection{Initial Setup of $\mathcal{FRSC}$s Contracts}
%We propose to initiate the contracts in our approach by some genesis value that enables even start.
To enable an even start, we propose to initiate $\mathcal{FRSC}$s of our approach by a genesis value.
The following formula calculates the genesis values per $\mathcal{FRSC}$ and initializes starting state of $\mathcal{FRSC}s_{[0]}$:
\begin{equation} \label{eq:setup}
	\{\mathcal{FRSC}_{[0]}^{x}(\nu, \lambda, \rho)\ |\ \nu = \overline{fees} * \mathbb{C} * \rho * \lambda\},
\end{equation}
where $\overline{fees}$ is the expected average of incoming fees.

==> sec/relatedwork.tex <==
The work of Carlsten et al.~\cite{carlsten2016instability} is the inspiration for our paper, which for the first time describes undercutting attacks arising from the exponential distribution of block creation time and significant differences in transaction fees.
The authors simulated Bitcoin under transaction-fee-based regime and found that there exist the minimal threshold of \textsc{Default-Compliant} miners equal to $66\%$. 

Gong et al.~\cite{gong2022towards} argue that using all accumulated fees in the mempool regardless of the block size limit is infeasible in practice and can inflate the profitability of undercutting that was originally described in~\cite{carlsten2016instability}.
Furthermore, Houy~\cite{houy2014economics} demonstrates that a constrain on the block size limit (thus the number of transactions) has economic importance and allows transaction fees not dropping to zero.
Therefore, Gong et al.~\cite{gong2022towards} model the profitability of undercutting with the block size limit presented, which bounds the claimable fees in a mining round.
The authors presented a countermeasure that selectively assembles transactions into the new block, while claiming fewer fees to avoid undercutting.
We argue that in contrast to our approach, this solution cannot be enforced by the consensus protocol, and thus might still enable undercutting to occur.

Zhou et al.~\cite{zhou2019robust} deal with the problem of a mining gap, which is more significant when the throughput of blockchain is high. 
Therefore, the authors propose the self-adaptive algorithm to
adjust the block size every 1000 blocks and thus ensure that blocks have enough space to pack new transactions.
%However, this mechanism 

%However, this was not demonstrated in a game theoretic analysis.

%We think combined solution could be beneficial towards better avoidance of undercutting attack and also towards more sustainable transaction fee regime. 

%\ih{todo ~\cite{moser2015trends}}


Even though Bitcoin-NG~\cite{eyal2016bitcoin} proposes a new consensus mechanism, it also contains an idea of splitting the transaction fees between two entities -- the current leader and the the miner of block -- which should incentivize the miner to include blocks created by the leader.
However, Bitcoin-NG is in some sense centralized and therefore, undercutting attacks are not its subject.
%This is similar approach in a way, as we also leave the miner take only portion of the fees.
%However the main point of paper~\cite{eyal2016bitcoin} is to showcase a blockchain with some features of Bitcoin while being more scalable with smaller confirmation time.\ \\
